Black-Box Training Data Identification in GANs via Detector Networks

Since their inception Generative Adversarial Networks (GANs) have been popular generative models across images, audio, video, and tabular data. In this paper we study whether given access to a trained GAN, as well as fresh samples from the underlying distribution, if it is possible for an attacker to efficiently identify if a given point is a member of the GAN's training data. This is of interest for both reasons related to copyright, where a user may want to determine if their copyrighted data has been used to train a GAN, and in the study of data privacy, where the ability to detect training set membership is known as a membership inference attack. Unlike the majority of prior work this paper investigates the privacy implications of using GANs in black-box settings, where the attack only has access to samples from the generator, rather than access to the discriminator as well. We introduce a suite of membership inference attacks against GANs in the black-box setting and evaluate our attacks on image GANs trained on the CIFAR10 dataset and tabular GANs trained on genomic data. Our most successful attack, called The Detector, involve training a second network to score samples based on their likelihood of being generated by the GAN, as opposed to a fresh sample from the distribution. We prove under a simple model of the generator that the detector is an approximately optimal membership inference attack. Across a wide range of tabular and image datasets, attacks, and GAN architectures, we find that adversaries can orchestrate non-trivial privacy attacks when provided with access to samples from the generator. At the same time, the attack success achievable against GANs still appears to be lower compared to other generative and discriminative models; this leaves the intriguing open question of whether GANs are in fact more private, or if it is a matter of developing stronger attacks.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> related_work.tex <==

\section{Related Work}
\emph{Membership Inference Attacks} or MIAs were defined by \cite{homer} for genomic data, and formulated by \cite{shokri_membership_2017} against ML models. In membership inference, an adversary uses model access as well as some outside information to determine whether a candidate point $x$ is a member of the model training set. Standard MIAs typically exploit the intuition that a point $x$ is more likely to be a training point if the loss of the model evaluated at $x$ is small \cite{yeom_privacy_2018}, or in the white-box setting where they have access to the model's gradients, if the gradients are small \cite{shokgrad}, although other approaches that rely on a notion of self-influence \cite{self-mi} and distance to the model boundary have been proposed \cite{neel, pap}. The state of the art attack against discriminative classifiers, called LiRA \cite{firstprinciple}, approximates the likelihood ratio of the loss when $x$ is in the training set versus not in the training set, training additional shadow models to sample from these distributions. 

Assuming access to the discriminator's loss, as in \cite{LOGAN}, loss-based attacks are easily ported over to GANs. However, given that the discriminator is not required to sample from the generator once training is finished, there is no practical reason to assume that the adversary has access to the discriminator. \cite{LOGAN} find that by thresholding on the discriminator loss, TPR at FPR = $.2$ on DCGAN trained on $\cifar$ is a little under $.4$ when the target GAN is trained for $100$ epochs, but goes up to almost $100\%$ after $200$ epochs, indicating severe over-fitting by the discriminator. When they employ a black-box attack, they are able to achieve TPR = $.37$ at FPR = $.2$.
We note that this is a less than $2$x improvement over baseline, even in the presence of potentially severe over-fitting during training. There have been a handful of recent papers that propose black-box attacks against generative models, nearly all of which rely on the heuristic that if a point is ``closer'' to generated samples that to random points from the distribution, it is more likely to be a training point \cite{Mi-montecarlo}\cite{chen_gan-leaks_2020}. The most closely related work to our detector methods is  ~\cite{refdata} who propose  a density-based model called DOMIAS, which infers membership by targeting local over-fitting of the generative models. Rather than train a detector network to classify whether samples are generated from the target GAN or the reference data, DOMIAS performs dimension reduction in order to directly estimate both densities, and then uses the ratio of the densities as a statistic for membership inference. We implement many of these methods in our experiments section, and summarize them in more detail in Appendix~\ref{sec:append_related}. 

 

==> tikzlibraryext.paths.ortho.code.tex <==
% Copyright 2022 by Qrrbrbirlbel
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%

%% For the operators r-lr, r-rl, r-ud and r-du we need to check after TikZ found r
\let\tikz@orig@rect\tikz@rect
\def\tikz@rect{\pgfutil@ifnextchar e\tikz@orig@rect\tikzext@tikz@r}
\def\tikzext@tikz@r -{%
  \pgfutil@ifnextchar l\tikzext@tikz@lr@lineto{%
    \pgfutil@ifnextchar r\tikzext@tikz@rl@lineto{%
      \pgfutil@ifnextchar u\tikzext@tikz@ud@lineto{%
        \pgfutil@ifnextchar d\tikzext@tikz@du@lineto\tikz@expand
      }%
    }%
  }%
}
%% For the operator |-| we need to check after TikZ found |-
\let\tikz@orig@vh@lineto@next\tikz@vh@lineto@next
\def\tikz@vh@lineto@next{%
  \pgfutil@ifnextchar|{\expandafter\tikzext@tikz@vhv@lineto\pgfutil@gobble}%
    {\pgfutil@ifnextchar\tikz@activebar{\expandafter\tikzext@tikz@vhv@lineto\pgfutil@gobble}%
      {\tikz@orig@vh@lineto@next}}}
%% For the operator -|- we need to check after TikZ found -|
\let\tikz@orig@hv@lineto\tikz@hv@lineto
\def\tikz@hv@lineto{%
  \pgfutil@ifnextchar-{\expandafter\tikzext@tikz@hvh@lineto\pgfutil@gobble}%
    {\tikz@orig@hv@lineto}}

%% |-|[<opts>] and -|-[<opts>] are allowed
\def\tikzext@tikz@vhv@lineto{\pgfutil@ifnextchar[{\tikzext@tikz@collect@hvvh@options\tikzext@tikz@vhv@lineto@next}{\tikzext@tikz@collect@hvvh@options\tikzext@tikz@vhv@lineto@next[]}}
\def\tikzext@tikz@hvh@lineto{\pgfutil@ifnextchar[{\tikzext@tikz@collect@hvvh@options\tikzext@tikz@hvh@lineto@next}{\tikzext@tikz@collect@hvvh@options\tikzext@tikz@hvh@lineto@next[]}}

%% r-rl[<opts>], r-lr[<opts>], etc.
\def\tikzext@tikz@rl@lineto rl{\pgfutil@ifnextchar[{\tikzext@tikz@collect@hvvh@options\tikzext@tikz@rl@lineto@next}{\tikzext@tikz@collect@hvvh@options\tikzext@tikz@rl@lineto@next[]}}
\def\tikzext@tikz@lr@lineto lr{\pgfutil@ifnextchar[{\tikzext@tikz@collect@hvvh@options\tikzext@tikz@lr@lineto@next}{\tikzext@tikz@collect@hvvh@options\tikzext@tikz@lr@lineto@next[]}}
\def\tikzext@tikz@du@lineto du{\pgfutil@ifnextchar[{\tikzext@tikz@collect@hvvh@options\tikzext@tikz@du@lineto@next}{\tikzext@tikz@collect@hvvh@options\tikzext@tikz@du@lineto@next[]}}
\def\tikzext@tikz@ud@lineto ud{\pgfutil@ifnextchar[{\tikzext@tikz@collect@hvvh@options\tikzext@tikz@ud@lineto@next}{\tikzext@tikz@collect@hvvh@options\tikzext@tikz@ud@lineto@next[]}}

%% TikZ interjects are done, the rest is independent:


\newdimen\tikzext@tikz@udlr@distance
\newdimen\tikzext@tikz@hvvh@distance
\newif\iftikzext@tikz@hvvh@middle         % checks whether spacing = 0 was selected
\newif\iftikzext@tikz@hvvh@fromcenter
\newif\iftikzext@ortho@preflush
\tikzext@ortho@preflushtrue

%%% HVVH/UDLR
\tikzset{%
  ortho/.code=\pgfqkeys{/tikz/ortho}{#1},
  hvvh/.code=\pgfqkeys{/tikz/ortho}{#1},%
  udlr/.code=\pgfqkeys{/tikz/ortho}{#1},%
  ortho/.search also=/tikz,
  ortho/middle 0 to 1/.style={/tikz/ortho/spacing=0},%
  ortho/from center/.is if=tikzext@tikz@hvvh@fromcenter,%
  ortho/spacing/.code=% spacing = 0 means that the middle part are the pos-itions 0 to 1,
  %                                           the first part is -1 to 0, the last part is to 2
    \pgfmathint{#1}\let\tikzext@tikz@hvvh@timing@parts\pgfmathresult% in case they are calculations to be done
    \ifcase\tikzext@tikz@hvvh@timing@parts\relax
      \tikzext@tikz@hvvh@middletrue
      \def\tikzext@tikz@hvvh@timing@parts{1}%
      \def\tikzext@tikz@hvvh@timing@first{0}%
      \def\tikzext@tikz@hvvh@timing@last{1}%
      \def\tikzext@tikz@hvvh@timing@subtr{0}%
      \def\tikzext@tikz@hvvh@timing@factor{1}%
    \else            % in all other cases n > 0 the kinks are at pos = 1/n and (n - 1)/n
      \tikzext@tikz@hvvh@middlefalse
      \pgfmathreciprocal{#1}\let\tikzext@tikz@hvvh@timing@first\pgfmathresult
      \pgfmathsetmacro\tikzext@tikz@hvvh@timing@last{1-\pgfmathresult}%
      \pgfmathreciprocal{#1-2}%
      \let\tikzext@tikz@hvvh@timing@subtr\pgfmathresult
      \pgfmathsetmacro\tikzext@tikz@hvvh@timing@factor{1+2*\pgfmathresult}%
    \fi,%
  ortho/ratio/.code=\pgfmathsetmacro\tikzext@tikz@hvvh@ratio{#1},%
  % TODO: not possible to do distance in TikZ coordinate system
  ortho/distance/.code=\pgfmathsetlength\tikzext@tikz@hvvh@distance{#1}\let\tikzext@tikz@hvvh@ratio\pgfutil@empty,%
  ortho/udlr distance/.style={%
    /tikz/ortho/ud distance={#1},%
    /tikz/ortho/du distance={#1},%
    /tikz/ortho/lr distance={#1},%
    /tikz/ortho/rl distance={#1}},%
  ortho/ud distance/.initial=+.5cm,%
  ortho/du distance/.initial=+.5cm,%
  ortho/lr distance/.initial=+.5cm,%
  ortho/rl distance/.initial=+.5cm,%
  ortho/ratio=.5,% default value
  ortho/spacing=4,% default value
}%

%BEGIN_FOLD Timer
\def\tikz@timer@hvhline{%
  \pgf@process{\tikz@timer@start}\pgf@ya\pgf@y
  \pgf@process{\tikz@timer@end}\pgf@yc\pgf@y
  \pgf@process{\tikz@timer@middle}\pgf@xb\tikz@time pt%
  \ifdim\tikz@time pt<\tikzext@tikz@hvvh@timing@first pt% first quarter
    \iftikzext@tikz@hvvh@middle
      \advance\pgf@xb1pt%
    \else
      \pgf@xb\tikzext@tikz@hvvh@timing@parts\pgf@xb
    \fi
    \edef\tikz@marshal{\noexpand\pgftransformlineattime{\pgf@sys@tonumber{\pgf@xb}}{\noexpand\tikz@timer@start}{%
        \noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@ya}}}%
  \else
    \ifdim\tikz@time pt>\tikzext@tikz@hvvh@timing@last pt% last quarter
      \iftikzext@tikz@hvvh@middle
        \advance\pgf@xb-1pt%
      \else
        \pgf@xb\tikzext@tikz@hvvh@timing@parts\pgf@xb
      \fi
      \advance\pgf@xb\dimexpr-\tikzext@tikz@hvvh@timing@parts pt+1pt\relax%
      \edef\tikz@marshal{\noexpand\pgftransformlineattime{\pgf@sys@tonumber{\pgf@xb}}%
        {\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@yc}}{\noexpand\tikz@timer@end}}%
    \else% middle half
      \pgf@xb\tikzext@tikz@hvvh@timing@factor\pgf@xb%
      \advance\pgf@xb-\tikzext@tikz@hvvh@timing@subtr pt%
      \edef\tikz@marshal{\noexpand\pgftransformlineattime{\pgf@sys@tonumber{\pgf@xb}}%
        {\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@ya}}{\noexpand\tikz@timer@middle}}%
    \fi\fi\tikz@marshal}
\def\tikz@timer@vhvline{%
  \pgf@process{\tikz@timer@start}\pgf@xa\pgf@x
  \pgf@process{\tikz@timer@end}\pgf@xc\pgf@x
  \pgf@process{\tikz@timer@middle}\pgf@xb\tikz@time pt%
  \ifdim\tikz@time pt<\tikzext@tikz@hvvh@timing@first pt% first quarter
    \iftikzext@tikz@hvvh@middle
      \advance\pgf@xb1pt%
    \else
      \pgf@xb\tikzext@tikz@hvvh@timing@parts\pgf@xb
    \fi
    \edef\tikz@marshal{\noexpand\pgftransformlineattime{\pgf@sys@tonumber{\pgf@xb}}{\noexpand\tikz@timer@start}{%
        \noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@y}}}%
  \else
    \ifdim\tikz@time pt>\tikzext@tikz@hvvh@timing@last pt% last quarter
    \iftikzext@tikz@hvvh@middle
      \advance\pgf@xb-1pt%
    \else
      \pgf@xb\tikzext@tikz@hvvh@timing@parts\pgf@xb
    \fi
      \advance\pgf@xb by\dimexpr-\tikzext@tikz@hvvh@timing@parts pt+1pt\relax%
      \edef\tikz@marshal{\noexpand\pgftransformlineattime{\pgf@sys@tonumber{\pgf@xb}}%
        {\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@y}}{\noexpand\tikz@timer@end}}%
    \else% middle half
      \pgf@xb=\tikzext@tikz@hvvh@timing@factor\pgf@xb
      \advance\pgf@xb by-\tikzext@tikz@hvvh@timing@subtr pt%
      \edef\tikz@marshal{\noexpand\pgftransformlineattime{\pgf@sys@tonumber{\pgf@xb}}%
        {\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@y}}{\noexpand\tikz@timer@middle}}%
      \fi\fi\tikz@marshal}%

%% collect options and nodes, coordinates and pics onpath
\let\tikz@hvvh@currentoption\pgfutil@empty
\def\tikzext@tikz@collect@hvvh@options#1[#2]{\edef\tikz@hvvh@currentoption{#2}#1}
\def\tikzext@tikz@hvh@lineto@next{%
  \pgfutil@ifnextchar n{\tikz@collect@label@onpath\tikzext@tikz@hvh@lineto@next}
    {\pgfutil@ifnextchar c{\tikz@collect@coordinate@onpath\tikzext@tikz@hvh@lineto@next}%
      {\pgfutil@ifnextchar p{\tikz@collect@pic@onpath\tikzext@tikz@hvh@lineto@next}{\tikz@scan@one@point\tikzext@tikz@@hvh@lineto}}}}%
\def\tikzext@tikz@vhv@lineto@next{%
  \pgfutil@ifnextchar n{\tikz@collect@label@onpath\tikzext@tikz@vhv@lineto@next}
    {\pgfutil@ifnextchar c{\tikz@collect@coordinate@onpath\tikzext@tikz@vhv@lineto@next}%
      {\pgfutil@ifnextchar p{\tikz@collect@pic@onpath\tikzext@tikz@vhv@lineto@next}{\tikz@scan@one@point\tikzext@tikz@@vhv@lineto}}}}%
\def\tikzext@tikz@ud@lineto@next{%
  \pgfutil@ifnextchar n{\tikz@collect@label@onpath\tikzext@tikz@ud@lineto@next}
    {\pgfutil@ifnextchar c{\tikz@collect@coordinate@onpath\tikzext@tikz@ud@lineto@next}
      {\pgfutil@ifnextchar p{\tikz@collect@pic@onpath\tikzext@tikz@ud@lineto@next}{\tikz@scan@one@point\tikzext@tikz@@ud@lineto}}}}%
\def\tikzext@tikz@du@lineto@next{%
  \pgfutil@ifnextchar n{\tikz@collect@label@onpath\tikzext@tikz@du@lineto@next}
    {\pgfutil@ifnextchar c{\tikz@collect@coordinate@onpath\tikzext@tikz@du@lineto@next}
      {\pgfutil@ifnextchar p{\tikz@collect@pic@onpath\tikzext@tikz@du@lineto@next}{\tikz@scan@one@point\tikzext@tikz@@du@lineto}}}}%
\def\tikzext@tikz@lr@lineto@next{%
  \pgfutil@ifnextchar n{\tikz@collect@label@onpath\tikzext@tikz@lr@lineto@next}
    {\pgfutil@ifnextchar c{\tikz@collect@coordinate@onpath\tikzext@tikz@lr@lineto@next}
      {\pgfutil@ifnextchar p{\tikz@collect@pic@onpath\tikzext@tikz@lr@lineto@next}{\tikz@scan@one@point\tikzext@tikz@@lr@lineto}}}}%
\def\tikzext@tikz@rl@lineto@next{%
  \pgfutil@ifnextchar n{\tikz@collect@label@onpath\tikzext@tikz@rl@lineto@next}
    {\pgfutil@ifnextchar c{\tikz@collect@coordinate@onpath\tikzext@tikz@rl@lineto@next}
      {\pgfutil@ifnextchar p{\tikz@collect@pic@onpath\tikzext@tikz@rl@lineto@next}{\tikz@scan@one@point\tikzext@tikz@@rl@lineto}}}}%

\def\tikz@do@hvvh#1#2#3#4#5{%
% #1 = first kink
% #2 = second kink
% #3 = end
% #4 = timer
% #5 = tikz@shapeborder@name
  \pgfpathlineto{#1}%
  \pgfpathlineto{#2}%
  \pgfpathlineto{#3}%
  \def\tikz@timer@middle{#2}%
  \def\tikz@timer@end{#3}%
  \let\tikz@timer#4
  \edef\pgf@temp{#5}%
  \ifx\pgf@temp\pgfutil@empty
    \let\tikz@moveto@waiting\relax
  \else
    \let\tikz@moveto@waiting\pgf@temp
  \fi
  \tikz@scan@next@command}%

%% -|- operator
\def\tikzext@tikz@@hvh@lineto#1{%
  \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  \pgf@xb=\tikz@lastx
  \pgf@xc=\tikz@lastx
  \pgf@yc=\tikz@lasty
  \tikz@make@last@position{#1}%
  \tikz@flush@moveto@toward{\pgfqpoint{\tikz@lastx}{\pgf@yc}}\pgf@xc\pgf@yc
  \begingroup
    \pgfqkeys{/tikz/ortho}{/tikz/style/.expand once=\tikz@hvvh@currentoption}%
    \iftikz@shapeborder
      \pgf@process{\pgfpointshapeborder{\tikz@shapeborder@name}{\pgfqpoint{\pgf@xb}{\tikz@lasty}}}%
      \iftikzext@tikz@hvvh@fromcenter
        \pgf@xc\pgf@xb
      \fi
      \pgfutil@ifxempty\tikzext@tikz@hvvh@ratio{%
        \ifdim\tikzext@tikz@hvvh@distance<0pt\relax
          \iftikzext@tikz@hvvh@fromcenter
            \pgf@xc\tikz@lastx
          \else
            \pgf@xc\pgf@x
          \fi
        \fi
        \ifdim\pgf@xb>\tikz@lastx
          \tikzext@tikz@hvvh@distance-\tikzext@tikz@hvvh@distance
        \fi
      }{%
        \iftikzext@tikz@hvvh@fromcenter
          \tikzext@tikz@hvvh@distance\tikz@lastx
        \else
          \tikzext@tikz@hvvh@distance\pgf@x
        \fi
        \advance\tikzext@tikz@hvvh@distance-\pgf@xc
        \tikzext@tikz@hvvh@distance\tikzext@tikz@hvvh@ratio\tikzext@tikz@hvvh@distance
      }%
      \advance\pgf@xc\tikzext@tikz@hvvh@distance
      \edef\pgf@tempa{\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
      \edef\pgf@tempb{\noexpand\pgfqpoint{\the\pgf@xc}{\the\tikz@lasty}}%
      \edef\pgf@temp{\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
    \else
      \let\tikz@shapeborder@name\pgfutil@empty
      \iftikzext@tikz@hvvh@fromcenter
        \pgf@xc\pgf@xb
      \fi
      \pgfutil@ifxempty\tikzext@tikz@hvvh@ratio{%
        \ifdim\tikzext@tikz@hvvh@distance<0pt\relax
          \pgf@xc\tikz@lastx
        \fi
        \ifdim\pgf@xb>\tikz@lastx
          \tikzext@tikz@hvvh@distance-\tikzext@tikz@hvvh@distance
        \fi
      }{%
        \tikzext@tikz@hvvh@distance\tikz@lastx
        \advance\tikzext@tikz@hvvh@distance-\pgf@xc
        \tikzext@tikz@hvvh@distance\tikzext@tikz@hvvh@ratio\tikzext@tikz@hvvh@distance
      }%
      \advance\pgf@xc\tikzext@tikz@hvvh@distance
      \edef\pgf@tempa{\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
      \edef\pgf@tempb{\noexpand\pgfqpoint{\the\pgf@xc}{\the\tikz@lasty}}%
      \edef\pgf@temp{\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
    \fi%
    \xdef\pgf@marshal{%
      \noexpand\tikz@do@hvvh
        {\expandafter\noexpand\pgf@tempa}%
        {\expandafter\noexpand\pgf@tempb}%
        {\expandafter\noexpand\pgf@temp}%
        {\noexpand\tikz@timer@hvhline}{\tikz@shapeborder@name}}%
  \endgroup
  \pgf@marshal}%

%% |-| operator
\def\tikzext@tikz@@vhv@lineto#1{%
  \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  \pgf@xc=\tikz@lastx
  \pgf@yb=\tikz@lasty
  \pgf@yc=\tikz@lasty
  \tikz@make@last@position{#1}%
  \tikz@flush@moveto@toward{\pgfqpoint{\pgf@xc}{\tikz@lasty}}\pgf@xc\pgf@yc
  \begingroup
    \pgfqkeys{/tikz/ortho}{/tikz/style/.expand once=\tikz@hvvh@currentoption}%
    \iftikz@shapeborder
      \pgf@process{\pgfpointshapeborder{\tikz@shapeborder@name}{\pgfqpoint{\tikz@lastx}{\pgf@yb}}}%
      \iftikzext@tikz@hvvh@fromcenter
        \pgf@yc\pgf@yb
      \fi
      \ifx\tikzext@tikz@hvvh@ratio\pgfutil@empty
        \ifdim\tikzext@tikz@hvvh@distance<0pt\relax
          \iftikzext@tikz@hvvh@fromcenter
            \pgf@yc\tikz@lasty
          \else
            \pgf@yc\pgf@y
          \fi
        \fi
        \ifdim\pgf@yb>\tikz@lasty
          \tikzext@tikz@hvvh@distance-\tikzext@tikz@hvvh@distance
        \fi
      \else
        \iftikzext@tikz@hvvh@fromcenter
          \tikzext@tikz@hvvh@distance\tikz@lasty
        \else
          \tikzext@tikz@hvvh@distance\pgf@y
        \fi
        \advance\tikzext@tikz@hvvh@distance-\pgf@yc
        \tikzext@tikz@hvvh@distance\tikzext@tikz@hvvh@ratio\tikzext@tikz@hvvh@distance
      \fi
      \advance\pgf@yc\tikzext@tikz@hvvh@distance
      \edef\pgf@tempa{\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
      \edef\pgf@tempb{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\pgf@yc}}%
      \edef\pgf@temp{\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
    \else
      \let\tikz@shapeborder@name\pgfutil@empty
      \iftikzext@tikz@hvvh@fromcenter
        \pgf@yc\pgf@yb
      \fi
      \ifx\tikzext@tikz@hvvh@ratio\pgfutil@empty
        \ifdim\tikzext@tikz@hvvh@distance<0pt\relax
          \pgf@yc\tikz@lasty
        \fi
        \ifdim\pgf@yb>\tikz@lasty
          \tikzext@tikz@hvvh@distance-\tikzext@tikz@hvvh@distance
        \fi
      \else
        \tikzext@tikz@hvvh@distance\tikz@lasty
        \advance\tikzext@tikz@hvvh@distance-\pgf@yc
        \tikzext@tikz@hvvh@distance\tikzext@tikz@hvvh@ratio\tikzext@tikz@hvvh@distance
      \fi
      \advance\pgf@yc\tikzext@tikz@hvvh@distance
      \edef\pgf@tempa{\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
      \edef\pgf@tempb{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\pgf@yc}}%
      \edef\pgf@temp{\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
    \fi%
    \xdef\pgf@marshal{%
      \noexpand\tikz@do@hvvh
        {\expandafter\noexpand\pgf@tempa}%
        {\expandafter\noexpand\pgf@tempb}%
        {\expandafter\noexpand\pgf@temp}%
        {\noexpand\tikz@timer@vhvline}{\tikz@shapeborder@name}}%
  \endgroup
  \pgf@marshal}%

%% r-ud operator
\def\tikzext@tikz@@ud@lineto#1{%
  \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  \pgf@xc\tikz@lastx
  \pgf@yb\tikz@lasty
  \advance\tikz@lasty1pt%
  \let\pgf@temp\tikz@moveto@waiting
  \tikz@flush@moveto@toward{\pgfqpoint{\tikz@lastx}{\tikz@lasty}}\pgf@xc\pgf@yc
  \tikz@make@last@position{#1}%
  \begingroup
    \pgfqkeys{/tikz/ortho}{/tikz/style/.expand once=\tikz@hvvh@currentoption}%
    \pgfmathsetlength\tikzext@tikz@udlr@distance{\pgfkeysvalueof{/tikz/ortho/ud distance}}%
    \iftikz@shapeborder
      \advance\pgf@y1pt%
      \pgf@process{\pgfpointshapeborder{\tikz@shapeborder@name}{\pgfqpoint{\pgf@x}{\pgf@y}}}%
      \iftikzext@tikz@hvvh@fromcenter
        \pgf@yc\pgf@yb
      \else\ifx\pgf@temp\relax
          \pgf@yc\pgf@yb
        \fi
      \fi
      \ifdim\pgf@yc<\pgf@y
        \iftikzext@tikz@hvvh@fromcenter
          \pgf@yc=\tikz@lasty
        \else
          \pgf@yc=\pgf@y
        \fi
      \fi
      \advance\pgf@yc\tikzext@tikz@udlr@distance
      \edef\pgf@temp{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
    \else
      \let\tikz@shapeborder@name\pgfutil@empty
      \ifx\pgf@temp\relax\else
        \iftikzext@tikz@hvvh@fromcenter\else
          \pgf@yb\pgf@yc
        \fi
      \fi
      \ifdim\pgf@yb<\tikz@lasty\pgf@yb\tikz@lasty\fi
      \advance\pgf@yb\tikzext@tikz@udlr@distance
      \pgf@yc\pgf@yb
      \edef\pgf@temp{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
    \fi
    \xdef\pgf@marshal{%
      \noexpand\tikz@do@hvvh
        {\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
        {\noexpand\pgfqpoint{\the\tikz@lastx}{\the\pgf@yc}}%
        {\expandafter\noexpand\pgf@temp}%
        {\noexpand\tikz@timer@vhvline}{\tikz@shapeborder@name}}%
  \endgroup
  \pgf@marshal}%

%% r-du operator
\def\tikzext@tikz@@du@lineto#1{%
  \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  \pgf@xc\tikz@lastx
  \pgf@yb\tikz@lasty
  \advance\tikz@lasty-1pt%
  \let\pgf@temp\tikz@moveto@waiting
  \tikz@flush@moveto@toward{\pgfqpoint{\tikz@lastx}{\tikz@lasty}}\pgf@xc\pgf@yc
  \tikz@make@last@position{#1}%
  \begingroup
    \pgfqkeys{/tikz/ortho}{/tikz/style/.expand once=\tikz@hvvh@currentoption}%
    \pgfmathsetlength\tikzext@tikz@udlr@distance{\pgfkeysvalueof{/tikz/ortho/du distance}}%
    \iftikz@shapeborder
      \advance\pgf@y-1pt%
      \pgf@process{\pgfpointshapeborder{\tikz@shapeborder@name}{\pgfqpoint{\pgf@x}{\pgf@y}}}%
      \iftikzext@tikz@hvvh@fromcenter
        \pgf@yc\pgf@yb
      \else\ifx\pgf@temp\relax
          \pgf@yc\pgf@yb
        \fi
      \fi
      \ifdim\pgf@yc>\pgf@y
        \iftikzext@tikz@hvvh@fromcenter
          \pgf@yc=\tikz@lasty
        \else
          \pgf@yc=\pgf@y
        \fi
      \fi
      \advance\pgf@yc-\tikzext@tikz@udlr@distance
      \edef\pgf@temp{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
    \else
      \let\tikz@shapeborder@name\pgfutil@empty
      \ifx\pgf@temp\relax\else
        \iftikzext@tikz@hvvh@fromcenter\else
          \pgf@yb\pgf@yc
        \fi
      \fi
      \ifdim\pgf@yb>\tikz@lasty\pgf@yb\tikz@lasty\fi
      \advance\pgf@yb-\tikzext@tikz@udlr@distance
      \pgf@yc\pgf@yb
      \edef\pgf@temp{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
    \fi
    \xdef\pgf@marshal{%
      \noexpand\tikz@do@hvvh
        {\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
        {\noexpand\pgfqpoint{\the\tikz@lastx}{\the\pgf@yc}}%
        {\expandafter\noexpand\pgf@temp}%
        {\noexpand\tikz@timer@vhvline}{\tikz@shapeborder@name}}%
  \endgroup
  \pgf@marshal}%

%% r-lr operator
\def\tikzext@tikz@@lr@lineto#1{%
  \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  \pgf@xb\tikz@lastx
  \pgf@yc\tikz@lasty
  \advance\tikz@lastx-1pt%
  \let\pgf@temp\tikz@moveto@waiting
  \tikz@flush@moveto@toward{\pgfqpoint{\tikz@lastx}{\tikz@lasty}}\pgf@xc\pgf@yc
  \tikz@make@last@position{#1}%
  \begingroup
    \pgfqkeys{/tikz/ortho}{/tikz/style/.expand once=\tikz@hvvh@currentoption}%
    \pgfmathsetlength\tikzext@tikz@udlr@distance{\pgfkeysvalueof{/tikz/ortho/lr distance}}%
    \iftikz@shapeborder
      \advance\pgf@x-1pt%
      \pgf@process{\pgfpointshapeborder{\tikz@shapeborder@name}{\pgfqpoint{\pgf@x}{\pgf@y}}}%
      \iftikzext@tikz@hvvh@fromcenter
        \pgf@xc\pgf@xb
      \else\ifx\pgf@temp\relax
          \pgf@xc\pgf@xb
        \fi
      \fi
      \ifdim\pgf@xc>\pgf@x
        \iftikzext@tikz@hvvh@fromcenter
          \pgf@xc=\tikz@lastx
        \else
          \pgf@xc=\pgf@x
        \fi
      \fi
      \advance\pgf@xc-\tikzext@tikz@udlr@distance
      \edef\pgf@temp{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
    \else
      \let\tikz@shapeborder@name\pgfutil@empty
      \ifx\pgf@temp\relax\else
        \iftikzext@tikz@hvvh@fromcenter\else
          \pgf@xb\pgf@xc
        \fi
      \fi
      \ifdim\pgf@xb>\tikz@lastx\pgf@xb\tikz@lastx\fi
      \advance\pgf@xb-\tikzext@tikz@udlr@distance
      \pgf@xc\pgf@xb
      \edef\pgf@temp{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
    \fi
    \xdef\pgf@marshal{%
      \noexpand\tikz@do@hvvh
        {\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
        {\noexpand\pgfqpoint{\the\pgf@xc}{\the\tikz@lasty}}%
        {\expandafter\noexpand\pgf@temp}%
        {\noexpand\tikz@timer@hvhline}{\tikz@shapeborder@name}}%
  \endgroup
  \pgf@marshal}%

%% r-rl operator
\def\tikzext@tikz@@rl@lineto#1{%
  \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  \pgf@xb\tikz@lastx
  \pgf@yc\tikz@lasty
  \advance\tikz@lastx1pt%
  \let\pgf@temp\tikz@moveto@waiting
  \tikz@flush@moveto@toward{\pgfqpoint{\tikz@lastx}{\tikz@lasty}}\pgf@xc\pgf@yc
  \tikz@make@last@position{#1}%
  \begingroup
    \pgfqkeys{/tikz/udlr}{/tikz/ortho/.expand once=\tikz@hvvh@currentoption}%
    \pgfmathsetlength\tikzext@tikz@udlr@distance{\pgfkeysvalueof{/tikz/ortho/rl distance}}%
    \iftikz@shapeborder%
      \advance\pgf@x1pt%
      \pgf@process{\pgfpointshapeborder{\tikz@shapeborder@name}{\pgfqpoint{\pgf@x}{\pgf@y}}}%
      \iftikzext@tikz@hvvh@fromcenter
        \pgf@xc\pgf@xb
      \else\ifx\pgf@temp\relax
          \pgf@xc\pgf@xb
        \fi
      \fi
      \ifdim\pgf@xc<\pgf@x
        \iftikzext@tikz@hvvh@fromcenter
          \pgf@xc=\tikz@lastx
        \else
          \pgf@xc=\pgf@x
        \fi
      \fi
      \advance\pgf@xc\tikzext@tikz@udlr@distance
      \edef\pgf@temp{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
    \else
      \let\tikz@shapeborder@name\pgfutil@empty%
      \ifx\pgf@temp\relax\else
        \iftikzext@tikz@hvvh@fromcenter\else
          \pgf@xb\pgf@xc
        \fi
      \fi
      \ifdim\pgf@xb<\tikz@lastx\pgf@xb\tikz@lastx\fi
      \advance\pgf@xb\tikzext@tikz@udlr@distance
      \pgf@xc\pgf@xb
      \edef\pgf@temp{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
    \fi
    \xdef\pgf@marshal{%
      \noexpand\tikz@do@hvvh
        {\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
        {\noexpand\pgfqpoint{\the\pgf@xc}{\the\tikz@lasty}}%
        {\expandafter\noexpand\pgf@temp}%
        {\noexpand\tikz@timer@hvhline}{\tikz@shapeborder@name}}%
  \endgroup
  \pgf@marshal}%

%% a few nice to haves, use with to or edge operator
\tikzset{
  node as new start/.is if=tikzext@ortho@preflush,
  node as new start,
  ortho/install shortcuts/.style={
    *|/.style={only vertical second={#1}},   *|/.default=,
    |*/.style={only vertical first={#1}},    |*/.default=,
    *-/.style={only horizontal second={#1}}, *-/.default=,
    -*/.style={only horizontal first={#1}},  -*/.default=,
    |-/.style={to path={|-(\tikztotarget)\tikztonodes}},
    -|/.style={to path={-|(\tikztotarget)\tikztonodes}},
    -|-/.style=/tikz/horizontal vertical horizontal,
    |-|/.style=/tikz/vertical horizontal vertical,
  },
  horizontal vertical/.style={to path={-| (\tikztotarget) \tikztonodes}},
  vertical horizontal/.style={to path={|- (\tikztotarget) \tikztonodes}},
  horizontal vertical horizontal/.style={to path={-|- (\tikztotarget) \tikztonodes}},
  vertical horizontal vertical/.style={to path={|-| (\tikztotarget) \tikztonodes}},
  only vertical second/.style={to path={
    \pgfextra
      \let\tikzext@ortho@anchor\pgfutil@empty
      \let\tikzext@origtotarget\pgfutil@empty
      \tikz@scan@one@point\pgfutil@firstofone(\tikztostart)\relax
      \iftikz@shapeborder
        \tikz@scan@one@point\pgfutil@firstofone(\tikztotarget)\relax
        \ifdim\pgf@y>\tikz@lasty\relax
          \edef\tikztostart{\tikztostart.north}%
          \iftikz@shapeborder\def\tikzext@ortho@anchor{.south}\fi
        \else
          \edef\tikztostart{\tikztostart.south}%
          \iftikz@shapeborder\def\tikzext@ortho@anchor{.north}\fi
        \fi
      \fi
      \def\tikz@tempa{#1}%
      \ifx\tikz@tempa\pgfutil@empty\else
        \let\tikzext@origtotarget\tikztotarget
        \edef\tikztotarget{[xshift={#1}]\tikztotarget\tikzext@ortho@anchor}%
      \fi
    \endpgfextra
    [insert path/.expanded={
      (perpendicular cs: horizontal line through={(\tikztostart)},
                         vertical line through={(\tikztotarget)}) -- (\tikztotarget)}] \tikztonodes
      \pgfextra
        \ifx\tikzext@origtotarget\pgfutil@empty\else
          \iftikzext@ortho@preflush(\tikzext@origtotarget)\fi\fi\endpgfextra}},
  only vertical second/.default=,
  only horizontal second/.style={to path={
    \pgfextra
      \let\tikzext@ortho@anchor\pgfutil@empty
      \let\tikzext@origtotarget\pgfutil@empty
      \tikz@scan@one@point\pgfutil@firstofone(\tikztostart)\relax
      \iftikz@shapeborder
        \tikz@scan@one@point\pgfutil@firstofone(\tikztotarget)\relax
        \ifdim\pgf@x>\tikz@lastx\relax
          \edef\tikztostart{\tikztostart.east}%
          \iftikz@shapeborder\def\tikzext@ortho@anchor{.west}\fi
        \else
          \edef\tikztostart{\tikztostart.west}%
          \iftikz@shapeborder\def\tikzext@ortho@anchor{.east}\fi
        \fi
      \fi
      \def\tikz@tempa{#1}%
      \ifx\tikz@tempa\pgfutil@empty\else
        \let\tikzext@origtotarget\tikztotarget
        \edef\tikztotarget{[yshift={#1}]\tikztotarget\tikzext@ortho@anchor}%
      \fi
    \endpgfextra
    [insert path/.expanded={
      (perpendicular cs: vertical line through={(\tikztostart)},
                         horizontal line through={(\tikztotarget)}) -- (\tikztotarget)}] \tikztonodes
    \pgfextra
      \ifx\tikzext@origtotarget\pgfutil@empty\else
        \iftikzext@ortho@preflush(\tikzext@origtotarget)\fi\fi\endpgfextra}},
  only horizontal second/.default=,
  only vertical first/.style={to path={
    \pgfextra
      \let\tikzext@ortho@anchor\pgfutil@empty
      \let\tikzext@origtotarget\pgfutil@empty
      \tikz@scan@one@point\pgfutil@firstofone(\tikztotarget)\relax
      \pgf@ya=\pgf@y
      \iftikz@shapeborder
        \let\tikzext@origtotarget\tikztotarget
        \tikz@scan@one@point\pgfutil@firstofone(\tikztostart)\relax
        \ifdim\pgf@ya>\tikz@lasty\relax
          \edef\tikztotarget{\tikztotarget.south}%
          \iftikz@shapeborder\def\tikzext@ortho@anchor{.north}\fi
        \else
          \edef\tikztotarget{\tikztotarget.north}%
          \iftikz@shapeborder\def\tikzext@ortho@anchor{.south}\fi
        \fi
      \fi
      \def\tikz@tempa{#1}%
      \ifx\tikz@tempa\pgfutil@empty\else
        \edef\tikztostart{[xshift={#1}]\tikztostart\tikzext@ortho@anchor}%
      \fi
    \endpgfextra
    [insert path/.expanded={(\tikztostart)}] 
    -- (perpendicular cs: vertical line through/.expanded={(\tikztostart)},
                        horizontal line through={(\tikztotarget)})
    \tikztonodes
    \pgfextra
      \ifx\tikzext@origtotarget\pgfutil@empty\else
        \iftikzext@ortho@preflush(\tikzext@origtotarget)\fi\fi\endpgfextra}},
  only vertical first/.default=,
  only horizontal first/.style={to path={
    \pgfextra
      \let\tikzext@ortho@anchor\pgfutil@empty
      \let\tikzext@origtotarget\pgfutil@empty
      \tikz@scan@one@point\pgfutil@firstofone(\tikztotarget)\relax
      \pgf@xa=\pgf@x
      \iftikz@shapeborder
        \let\tikzext@origtotarget\tikztotarget
        \tikz@scan@one@point\pgfutil@firstofone(\tikztostart)\relax
        \ifdim\pgf@xa>\tikz@lastx\relax
          \edef\tikztotarget{\tikztotarget.west}%
          \iftikz@shapeborder\def\tikzext@ortho@anchor{.east}\fi
        \else
          \edef\tikztotarget{\tikztotarget.east}%
          \iftikz@shapeborder\def\tikzext@ortho@anchor{.west}\fi
        \fi
      \fi
      \def\tikz@tempa{#1}%
      \ifx\tikz@tempa\pgfutil@empty\else
        \edef\tikztostart{[yshift={#1}]\tikztostart\tikzext@ortho@anchor}%
      \fi
    \endpgfextra
    [insert path/.expanded={(\tikztostart)}]
      -- (perpendicular cs: horizontal line through/.expanded={(\tikztostart)},
                              vertical line through={(\tikztotarget)})
    \tikztonodes \pgfextra
      \ifx\tikzext@origtotarget\pgfutil@empty\else
        \iftikzext@ortho@preflush(\tikzext@origtotarget)\fi\fi\endpgfextra}},
  only horizontal first/.default=,
  only vertical first to center/.style={to path={
      \pgfextra
        \let\tikzext@origtotarget\tikztotarget
      \endpgfextra
    (\tikztostart) -- (perpendicular cs: vertical line through={(\tikztostart)},
                                         horizontal line through={(\tikztotarget)})
    \tikztonodes \ifx\tikzext@origtotarget\pgfutil@empty\else\iftikzext@ortho@preflush(\tikzext@origtotarget)\fi\fi}},
  only horizontal first to center/.style={to path={
      \pgfextra
        \let\tikzext@origtotarget\tikztotarget
      \endpgfextra
    (\tikztostart) -- (perpendicular cs: horizontal line through={(\tikztostart)},
                                         vertical line through={(\tikztotarget)})
    \tikztonodes \ifx\tikzext@origtotarget\pgfutil@empty\else\iftikzext@ortho@preflush(\tikzext@origtotarget)\fi\fi}}%
}
\endinput
